On Euler systems and Nekov\'a\v{r}-Selmer complexes

We develop a theory of Euler and Kolyvagin systems relative to the Nekov\'{a}\v{r}--Selmer complexes of $p$-adic representations over local complete Gorenstein rings. This theory is both finer and requires fewer hypotheses than those of Mazur and Rubin over discrete valuation rings and of Sakamoto et al. over Gorenstein rings. In particular, given appropriate Euler systems, it allows one to study Selmer groups defined relative to Greenberg local conditions. As initial applications, we prove new cases of Kato's generalised Iwasawa main conjecture for both $\mathbb{Z}_p(a)$ and the $p$-adic Tate modules of rational elliptic curves, new cases of the Quillen--Lichtenbaum Conjecture, and a strengthening of existing results on the Birch--Swinnerton-Dyer Conjecture for CM elliptic curves.

==> preamble.tex <==

%%%packages - alphabetically
    \usepackage{aliascnt}
	\usepackage{amsmath}	
	\usepackage{amssymb}
	\usepackage{amsthm}
	\usepackage[british]{babel}
	\usepackage{bm}
	\usepackage{braket}
	\usepackage{comment}
	\usepackage{datetime}
	\usepackage{enumitem}
	\usepackage[inner=26mm, outer=26mm, 
	top=22mm, 
	bottom=28mm,
				a4paper]{geometry}
	\usepackage[framemethod=TikZ, roundcorner=1mm, linecolor=gray]{mdframed}
	\usepackage{tikz-cd}
  \usepackage[all]{xy}
  \SelectTips{cm}{10}
	\usepackage{url}
	\usepackage{stmaryrd}
	\usepackage{xcolor}
	\usepackage{mathdots}
	\usepackage{mathrsfs}
	\usepackage{mathtools}
	\usepackage{todonotes}

\DeclareMathAlphabet{\mathboondoxfrak}{U}{BOONDOX-frak}{m}{n}
\newcommand{\bfF}{\mathboondoxfrak{F}}
\newcommand{\ufF}{\underline{\fF}}
\newcommand{\scrF}{\mathscr{F}}

%%%%%%Title font
\RequirePackage{fix-cm}
\makeatletter
\newcommand\semiLARGE{\@setfontsize\semiLARGE{16.5}{16.5}}
\makeatother

% Redefine \part to produce inline "Part I. The general theory" with smaller font
\makeatletter
\renewcommand{\part}[1]{%
  \refstepcounter{part}% Increase part counter
  \addcontentsline{toc}{part}{\partname~\thepart.\ #1}% Add to TOC
  \vspace{2em}% Space before part title
  {\sffamily\semiLARGE\bfseries% Set font size and style here
    \partname~\thepart.\ #1\par}% Single-line output
  \vspace{1em}% Space after part title
}
\makeatother



%Tikz
\usepackage{tikz-cd, tikz-3dplot, pgfplots}
\usetikzlibrary{patterns, arrows, positioning, decorations.markings}
\tikzset{axis/.style={very thick, ->}}
\tikzset{
 		  every pin/.style={pin edge={<-}},
  		>=stealth,
   		flow/.style={decoration={markings,mark=at position #1 with {\arrow[black, 
			line width=1.3pt]{>}}},
       		postaction={decorate}},
   		flow/.default=0.5,
		flow_inv/.style={decoration={markings,mark=at position #1 with 
			{\arrow[black, line width=1.3pt]{<}}},
       		postaction={decorate}},
   		flow_inv/.default=0.5,
  		eigendirection/.style={dashed, grau, very thick}
  	}
	
	\tikzset{graph/.style={grau}}
	
\tikzset{
    slanted/.style={rotate=-90, anchor = south},
    slantedswap/.style={rotate=-90, anchor=north}
}


\usepackage{xpatch}
\xapptocmd\normalsize{%
 \abovedisplayskip=5pt plus 3pt minus 1pt
 \abovedisplayshortskip=3pt plus 2pt minus 2pt
 \belowdisplayskip=5pt plus 1pt minus 3pt
 \belowdisplayshortskip=3pt plus 2pt minus 2pt
}{}{}


%% Definition der Sätze und Co.
\newtheorem*{thmintro}{Theorem}
\newtheorem*{corintro}{Corollary}
      	%\renewcommand{\thethmintro}{\Alph{thmintro}}
	
	\newtheoremstyle{parenfirstplain}
  {\topsep}   % Space above
  {\topsep}   % Space below
  {}  % Body font
  {}          % Indent amount
  {\bfseries} % Theorem head font
  {.}          % Punctuation after theorem head
  { }         % Space after theorem head
  {\thmnumber{(#2)}\ \thmname{#1}\thmnote{~#3}} % <== Number first

\theoremstyle{parenfirstplain}
	\newtheorem*{thmplain}{Theorem}
    \numberwithin{equation}{section}
    \newtheorem{remark}[equation]{Remark}
	\newtheorem{remarks}[equation]{Remark}
    \newtheorem{hypothesis}[equation]{Hypothesis}
	\newtheorem{hypotheses}[equation]{Hypotheses}
    \newtheorem{hyp}[equation]{Hypothesis}
    \newtheorem{hyps}[equation]{Hypotheses}
    \newtheorem{example}[equation]{Example}
	\newtheorem{examples}[equation]{Examples}
    \newtheorem*{acknowledgments}{Acknowledgements}
    \newtheorem{bsp1}[equation]{Example}
	\newtheorem{bspe1}[equation]{Examples}
    \newtheorem{ex}[equation]{Exercise}
	\newtheorem{rk}[equation]{Remark}
    \newtheorem{observation}[equation]{Observation}
    \newtheorem{strategy}[equation]{Strategy}
	\newtheorem{caveat}[equation]{Caveat}

    	\newtheoremstyle{parenfirstit}
  {\topsep}   % Space above
  {\topsep}   % Space below
  {\itshape}  % Body font
  {}          % Indent amount
  {\bfseries} % Theorem head font
  {.}          % Punctuation after theorem head
  { }         % Space after theorem head
  {\thmnumber{(#2)}\,\thmname{#1}\thmnote{\,\normalfont (#3)}} % <== Number first
    
	\theoremstyle{parenfirstit}
	\newtheorem{theorem}{equation}[section]
    \newtheorem{thm}[equation]{Theorem}
	\newtheorem{condition}[equation]{Condition}
    \newtheorem{definition}[equation]{Definition}
	\newtheorem{question}[equation]{Question}
    \newtheorem{conj}[equation]{Conjecture}
	\newtheorem{prop}[equation]{Proposition}
	\newtheorem{cor}[equation]{Corollary}
	\newtheorem{lem}[equation]{Lemma}
	\newtheorem{lemma}[equation]{Lemma}
	\newtheorem{corollary}[equation]{Corollary}
	\newtheorem{proposition}[equation]{Proposition}
	\newtheorem{conjecture}[equation]{Conjecture}

    \swapnumbers
	\newcounter{Claim}
	\newtheorem{claim}[Claim]{Claim}

%    

%%Definitio of respective environments
	\newenvironment{bsp}
	{\begin{bsp1}}
	{  \end{bsp1}}
	 
	\newenvironment{bspe}
	{\begin{bspe1}
	\begin{liste}}
	{\end{liste}
	\end{bspe1}}

\setlist[enumerate]{topsep=2pt, itemsep=2pt, parsep=0pt}
\setlist[itemize]{topsep=2pt, itemsep=2pt, parsep=0pt}
	\newenvironment{liste}
	{\begin{enumerate}[label=(\alph*)]
	%\setlength{\itemsep}{3pt}
  %\setlength{\parskip}{0pt}
  %\setlength{\parsep}{0pt}
  }
	{\end{enumerate}}

 \newenvironment{romanliste}
	{\begin{enumerate}[label=(\roman*)]
	%\setlength{\itemsep}{3pt}
  %\setlength{\parskip}{0pt}
 % \setlength{\parsep}{0pt}
 }
	{\end{enumerate}}


	\newenvironment{cdiagram}
	{\begin{equation*} \begin{tikzcd}}
	{\end{tikzcd}\end{equation*}%
	}
	
	


%%Crazy Shortcuts - alphabetically
    \newcommand{\anti}{\mathrm{anti}}
	\renewcommand{\:}{\colon}
	\renewcommand{\a}{\mathfrak{a}}
	\newcommand{\bigO}{\mathcal{O}}
	\newcommand{\characteristic}{\operatorname{char}}
	\newcommand{\Char}{\operatorname{char}}
	\newcommand{\cl}{\operatorname{cl}}
	\newcommand{\C}{\mathbb{C}}
	\newcommand{\cM}{\mathcal{M}}
	\newcommand{\cX}{\mathcal{X}}
 \newcommand{\cP}{\mathcal{P}}
	\newcommand{\dd}{\mathrm{d}}
	\newcommand{\Eig}{\operatorname{Eig}}
	\renewcommand{\emptyset}{\varnothing}
	\renewcommand{\emph}[1]{\textit{\textbf{#1}}}
	\newcommand{\fL}{\mathfrak{L}}
 \newcommand{\fX}{\mathfrak{X}}
	\newcommand{\ff}{\mathfrak{f}}
    \newcommand{\fF}{\mathfrak{F}}
	\newcommand{\Fitt}{\operatorname{Fitt}}
	\newcommand{\Frob}{\mathrm{Frob}}
	\newcommand{\gal}[2]{\mathrm{Gal}( #1 / #2)}
	\renewcommand{\iff}{\quad \Leftrightarrow \quad}
	\newcommand{\id}{\mathrm{id}}
	\newcommand{\legendre}[2]{ \left( \frac{#1}{#2} \right)}
	 \newcommand{\Log}{\text{Log}} 
	 \newcommand{\N}{\mathbb{N}}
	\newcommand{\p}{\mathfrak{p}}
	\renewcommand{\P}{\mathfrak{P}}
	\newcommand{\m}{\mathfrak{m}}
 \newcommand{\n}{\mathfrak{n}}
	\newcommand{\q}{\mathfrak{q}}
	\newcommand{\Q}{\mathbb{Q}}
	\newcommand{\Ord}{\mathrm{Ord}}
	\newcommand{\ord}{\mathrm{ord}}
 \newcommand{\order}{\mathrm{order}}
	\newcommand{\R}{\mathbb{R}}
	\renewcommand{\Re}{\operatorname{Re}}
	\newcommand{\Res}[2]{\operatorname{Res}\left (#1; \, #2 \right )}	
	\newcommand{\Rec}{\mathrm{Rec}}
    \newcommand{\Rlim}[1]{
    \mathchoice{
    \underset{\overleftarrow{#1}}{
    \operatorname{Rlim}\,}}
    {\underleftarrow{\operatorname{Rlim}}_{#1}}
    {\underleftarrow{\operatorname{Rlim}}_{#1}}
    {\underleftarrow{\operatorname{Rlim}}_{#1}}
    }
	\newcommand{\rec}{\mathrm{rec}}
	\newcommand{\so}{\quad \Rightarrow \quad}
	\newcommand{\sgn}{\operatorname{sgn}}
	\renewcommand{\ord}{\operatorname{ord}}
	\newcommand{\Stab}{\mathrm{Stab}}	
	\newcommand{\svector}[3]{\begin{pmatrix} #1 \\ #2 \\ #3 \end{pmatrix}}
 \newcommand{\tr}{\mathrm{tr}}
 \newcommand{\fs}{\mathrm{fs}}
	\newcommand{\UN}{\mathrm{UN}}
	\newcommand{\Z}{\mathbb{Z}}
	\newcommand{\fin}{\mathrm{fin}}
\DeclareMathOperator{\length}{length}
	
	
	
	%%%verlinktes toc
	\PassOptionsToPackage{hyphens}{url}
\usepackage[colorlinks,
pdfpagelabels,
pdfstartview = FitH,
bookmarksopen = true,
bookmarksnumbered = true,
linkcolor = black,
plainpages = false,
hypertexnames = false,
citecolor = black, urlcolor=black]{hyperref}

\newcommand{\nocontentsline}[3]{}
\newcommand{\tocless}[2]{\bgroup\let\addcontentsline=\nocontentsline#1{#2}\egroup}

%%%%%%%%%label text

\newcounter{mylabelcounter}


\makeatletter
\newcommand{\labeltext}[2]{%
  \phantomsection%
  \refstepcounter{mylabelcounter}%
  #1%
  \def\@currentlabelname{#1}% Store the name for \nameref
  \label{#2}%
}
\makeatother


%bunch of environment definitions

\font\russ=wncyr10 \font\Russ=wncyr10   scaled\magstep 1
\def\sha{\hbox{\russ\char88}}
\def\CYRBE{\hbox{\russ B}}

%%More crazy shortcuts
\newcommand{\Abar}{{\bar A}}
\newcommand{\cAbar}{{\bar \cA}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\Tbar}{{\overline{T}}}
\newcommand{\cTbar}{{\overline{\cT}}}

\newcommand{\vir}[1]{{\bf [} #1{\bf ]}}
\newcommand{\eins}{\boldsymbol{1}}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Cl}{Cl}
\DeclareMathOperator{\Det}{Det}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\Gal}{Gal}
\DeclareMathOperator{\Ho}{H}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\ind}{ind}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\RHom}{RHom}
\newcommand{\RGamma}{\mathrm{R}\Gamma}
\newcommand{\TNC}{\mathrm{TNC}}

\newcommand{\CC}{\mathbb{C}}
\newcommand{\bc}{\mathbb{C}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\NN}{\mathrm{N}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\br}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\bfp}{\mathbb{F}}
\newcommand{\ZG}{\mathbb{Z}[G]}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\G}{\mathcal{G}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\cS}{\mathcal{S}}

\newcommand{\frakm}{\mathfrak{m}}
\newcommand{\frp}{\mathfrak{p}}
\newcommand{\frakA}{\mathfrak{A}}
\newcommand{\fq}{\mathfrak{q}}
\newcommand{\fp}{\mathfrak{p}}

\newcommand{\fa}{\mathfrak{a}}
\newcommand{\fb}{\mathfrak{b}}
\newcommand{\fd}{\mathfrak{d}}
\newcommand{\fn}{\mathfrak{n}}

\newcommand{\arch}{\mathrm{arch}}
\DeclareMathOperator{\aug}{aug}
\DeclareMathOperator{\Br}{Br}
\DeclareMathOperator{\centre}{Z}
\newcommand{\cok}{\text{cok}}
\newcommand{\cone}{\mathrm{cone}}
\newcommand{\dR}{\mathrm{dR}}
\newcommand{\et}{\mathrm{\acute et}}
\newcommand{\Eul}{\mathrm{Eul}}
\newcommand{\even}{\mathrm{ev}}
\newcommand{\finite}{\mathrm{finite}}
\newcommand{\glob}{\mathrm{glob}}
\newcommand{\Imag}{\mathbf{I}}
\DeclareMathOperator{\inv}{inv}
\newcommand{\Irr}{\mathrm{Irr}}
\newcommand{\loc}{\mathrm{loc}}
\newcommand{\nr}{\mathrm{Nrd}}
\newcommand{\odd}{\mathrm{od}}
\newcommand{\old}{\mathrm{old}}
\newcommand{\perf}{\mathrm{p}}
\newcommand{\quot}{\mathrm{q}}
\newcommand{\real}{\mathrm{Re}}
\newcommand{\Real}{\mathbf{R}}
\newcommand{\Reg}{\mathrm{Reg}}
\newcommand{\Sel}{\mathrm{Sel}}
\newcommand{\tors}{\mathrm{tors}}
\newcommand{\pr}{\mathrm{pr}}
\newcommand{\Ann}{\mathrm{Ann}}
\newcommand{\bz}{\mathbb{Z}}
\newcommand{\La}{\Lambda}
\newcommand{\bq}{\mathbb{Q}}
\newcommand{\fz}{\mathfrak{z}}
\def\bigcapp{\raise1ex\hbox{\rotatebox{180}{$\biguplus$}}}
 \def\bigcappd{\raise1ex\hbox{\rotatebox{180}{$\displaystyle\biguplus$}}}


 \newcommand{\ES}{\mathrm{ES}}
  \newcommand{\Ev}{\mathrm{Ev}}
  \newcommand{\KS}{\mathrm{KS}}
  \renewcommand{\SS}{\mathrm{StS}}
  \newcommand{\RES}{\mathrm{RES}}
 \newcommand{\VS}{\mathrm{VS}}
 \newcommand{\cyc}{\mathrm{cyc}}
 \newcommand{\cV}{\mathcal{V}}
 \newcommand{\tor}{\mathrm{tor}}
 \newcommand{\tf}{\mathrm{tf}}
 \newcommand{\cE}{\mathcal{E}}
 \newcommand{\cC}{\mathcal{C}}
  \newcommand{\cN}{\mathcal{N}}
 \newcommand{\cL}{\mathcal{L}}
 \newcommand{\Fr}{\mathrm{Fr}}
 \newcommand{\cR}{\mathcal{R}}
 \newcommand{\ram}{\mathrm{ram}}
 \newcommand{\cores}{\mathrm{cores}}
 \newcommand{\bidual}{\bigcap\nolimits}
\newcommand{\exprod}{\bigwedge\nolimits}
\newcommand{\rank}{\mathrm{rk}}
\newcommand{\spc}{\mathrm{split}}
\renewcommand{\split}{\mathrm{s}}
\newcommand{\NS}{\mathrm{NS}}
\newcommand{\Iw}{\mathrm{Iw}}
\newcommand{\Cyc}{\mathrm{Cyc}}
\newcommand{\cchar}{\mathrm{char}}
\newcommand{\unr}{\mathrm{nr}}
 \newcommand{\cY}{\mathcal{Y}}
 
  \tikzset{
    rotated/.style={rotate=-90, anchor = south},
    rotatedswap/.style={rotate=-90, anchor=north, outer sep=0.75mm}
}

\newcommand{\Be}{\mbox{\usefont{T2A}{\rmdefault}{m}{n}\CYRBE}}

\newcommand{\bLambda}{{\mathpalette\makebLambda\relax}}
\newcommand{\makebLambda}[2]{%
  \raisebox{\depth}{\scalebox{1}[-1]{$\mathsurround=0pt#1\mathbb{V}$}}%
}


\newcommand{\straightLambda}{{\mathpalette\makestraightLambda\relax}}
\newcommand{\makestraightLambda}[2]{%
  \raisebox{\depth}{\scalebox{1}[-1]{$\mathsurround=0pt#1\text{V}$}}%
}

\usepackage{dsfont}
\renewcommand{\mathbb}{\mathds}
\newcommand{\rm}{\textrm}
	\tikzcdset{
  cells={font=\everymath\expandafter{\the\everymath\displaystyle}},
}


	\usepackage{tocloft}

\renewcommand\cftsecfont{\normalfont}
\renewcommand\cftsecpagefont{\normalfont}
\renewcommand{\cftsecleader}{\cftdotfill{\cftsecdotsep}}
\renewcommand\cftsecdotsep{\cftdot}
\renewcommand\cftsubsecdotsep{\cftdot}


\newcommand{\eullim}[2]{\mathchoice{\underset{#1}{\underleftarrow{\mathrm{elim}}^{#2}} \,}{{\underleftarrow{\mathrm{elim}}}^{#2}_{#1}}{{\underleftarrow{\mathrm{elim}}}^{#2}_{#1}}{{\underleftarrow{\mathrm{elim}}}^{#2}_{#1}}}

\newcommand{\resprod}[1]{\mathbin{
		\ooalign{
		 \raisebox{-1.57ex}{\scalebox{1.5}
			{$-$}
			}
			\cr\hidewidth\raisebox{.0ex}{
			%\scalebox{2}
			{$\displaystyle \prod_{#1 } $}
			}
			\hidewidth
			}
			}}
	\newcommand{\resprodt}{\mathbin{\ooalign{\raisebox{-.95ex}{$-$}
						\cr\hidewidth\raisebox{.2ex}{
						%\scalebox{2}
						{$\prod$}}
						\hidewidth
						}}}		


\makeatletter
\newcounter{savesection}
\newcounter{apdxsection}
\renewcommand\appendix{\par
  \setcounter{savesection}{\value{section}}%
  \setcounter{section}{\value{apdxsection}}%
  \setcounter{subsection}{0}%
  \gdef\thesection{\@Alph\c@section}}
\newcommand\unappendix{\par
  \setcounter{apdxsection}{\value{section}}%
  \setcounter{section}{\value{savesection}}%
  \setcounter{subsection}{0}%
  \gdef\thesection{\@arabic\c@section}}
\makeatother
                        
